Recommending Analogical APIs via Knowledge Graph Embedding

Library migration, which re-implements the same software behavior by using a different library instead of using the current one, has been widely observed in software evolution. One essential part of library migration is to find an analogical API that could provide the same functionality as current ones. However, given the large number of libraries/APIs, manually finding an analogical API could be very time-consuming and error-prone. Researchers have developed multiple automated analogical API recommendation techniques. Documentation-based methods have particularly attracted significant interest. Despite their potential, these methods have limitations, such as a lack of comprehensive semantic understanding in documentation and scalability challenges. In this work, we propose KGE4AR, a novel documentation-based approach that leverages knowledge graph (KG) embedding to recommend analogical APIs during library migration. Specifically, KGE4AR proposes a novel unified API KG to comprehensively and structurally represent three types of knowledge in documentation, which can better capture the high-level semantics. Moreover, KGE4AR then proposes to embed the unified API KG into vectors, enabling more effective and scalable similarity calculation. We build KGE4AR' s unified API KG for 35,773 Java libraries and assess it in two API recommendation scenarios: with and without target libraries. Our results show that KGE4AR substantially outperforms state-of-the-art documentation-based techniques in both evaluation scenarios in terms of all metrics (e.g., 47.1%-143.0% and 11.7%-80.6% MRR improvements in each scenario). Additionally, we explore KGE4AR' s scalability, confirming its effective scaling with the growing number of libraries.

==> candidate_filter.tex <==
We found that there are a large number of API methods from the same library and the same class in the returned results.
In order to make the results more diverse, we filter the candidates by only keep at most the top-$M$ methods of the same library and at most the top-$N$ of the same class.
In our implementation, $M$ and $N$ are set as to 15 and 3, respectively.

==> discussion.tex <==
Our current implementation of \app only supports Java libraries, but it can be easily extended to support libraries of other object-oriented languages.
To support a new language, we only need to replace the static analysis tool used to extract API elements and structural relations.
Moreover, we can even construct a cross-language API KG which includes libraries of different languages based on the same schema (see Figure~\ref{fig:kgschema}).
Based on the APK KG, we can support cross-language API mapping.
\yiling{This paragraph could be merged with the last paragraph in threats section.}


When planning library migration, the developer usually needs to consider a set of source API methods as a whole by finding a target library that can provide all the required analogical API methods.
\app can support this requirement by recommending target libraries and the corresponding API methods based on the combination of the recommendations for individual source API methods.
The developer then can choose one or multiple target libraries that have good overall coverage of the required analogical API methods.

\yiling{Currently I didn't find the necessaity of the discussion section.}

%\todo{Move RQ1 here.}

==> evaluation_bak.tex <==
We implement \app and construct an API KG for Java libraries.
To prepare JAR files as input, we first get the metadata (\eg groupId and artifactId) of a list of Java libraries according to the Libraries.io dataset \cite{libariesiodata} (last updated in January 2020).
Then, we download the latest version of JAR files (as of August 11, 2022) from the Maven Central Repository, resulting in 35,773 JAR files.
We construct an API KG with 72,242,099 entities and 289,122,265 relations based on these JAR files,
Among them, 59,155,631 entities are API elements, 5,210,925 entities are functionality elements, and 5,660,553 entities are concepts.
Table~\ref{table:kg_statistics} shows the details of each entity type.
Further, we train the KG embedding model based on ComplEx with a logistic loss.
%The produced KG embeddings of all entities are stored in a vector database, \ie Milvus~\cite{milvus}.
%The API KG and the corresponding KG embedding model are released in our replication package~\cite{replication_package}.
%The weights of these similarities for re-ranking candidate API methods (see Eq.~\ref{eq:sim:sum}) are important for \app.
%We tune these weights on a benchmark and the best configuration is that $W_{m}=0.05$, $W_{func}=0.95$, $W_{obj}=0.8$, $W_{it}=0.25$, $W_{iv}=0.05$, $W_{ot}=0.05$, and $W_{neig}=0.95$ (see Section~\ref{sec:rq3}).
% based on the metadata by using the REST APIs~\cite{mavenapi}.
%Note that we download the source JAR files which contain only source code files, \ie .java files.
%The comments in source JAR files are reserved as they are useful in the following KG construction.
%The API KG is stored in a graph database, \ie Neo4j~\cite{neo4j}.
\begin{table}[]
	\footnotesize
	\centering
	\vspace{-6mm}
	\caption{Statistics of Resulting API KG}
	\vspace{-3mm}
	\label{table:kg_statistics}
	\begin{tabular}{|c|c|c|c|}
		\hline
		Type          & Number & Type          & Number \\ \hline
		Library &   35,773 & Return Value          & 15,451,223   \\ \hline
		Package &   229,061 & Abstract Parameter & 1,892,120  \\ \hline
		Class &   3,090,537 & Functionality Expression &   5,200,297  \\ \hline
		Interface &    281,854 &   Functionality Category &  89    \\ \hline
		Field &   6,232,643   & Functionality Verb  &  10,016  \\ \hline
		Method &    15,441,057  & Phrase Pattern &  523\\ \hline
		Parameter          & 16,501,363&  Concept &    5,660,553 \\ \hline
	\end{tabular}
\vspace{-7mm}
\end{table}

To evaluate the effectiveness and scalability of \app, we conduct a series of experiments by answering the following research questions. 

\textbf{RQ1 (Effectiveness with Target Libraries)}: How does \app perform at inferring analogical API methods with a given target library compared to the baselines? 

\textbf{RQ2 (Effectiveness without Target Libraries)}: How does \app perform at inferring analogical API methods without a given target library compared to the baselines? 

\textbf{RQ3 (Factor Impact)}: How do different factors in \app (i.e., the KG embedding models, knowledge types, and similarity types and weights) affect the effectiveness of \app? 

\textbf{RQ4 (Scalability)}: How well can \app scale with the increase of the number of libraries?

\subsection{RQ1: Effectiveness with Given Target Libraries}
\label{sec:rq1}
\input{rq1}

\subsection{RQ2: Effectiveness without Given Target Libraries}
\label{sec:rq2}
\input{rq2}

\subsection{RQ3: Factor Impact}
\label{sec:rq3}
\input{rq3}

\subsection{RQ4: Scalability}
\label{sec:rq4}
\input{rq4}

\subsection{Threats to Validity}
\label{sec:threats}
\input{threats}


==> introduction_bak.tex <==
Third-party libraries have been widely used in modern software development for improving the quality and productivity and reducing the time to market~\cite{softw94libreuse,ese07libreuse,fse12libmigration,ese18libmigration}.
With the rise of code hosting platforms (\eg GitHub~\cite{github}) and package hosting platforms (\eg Maven Central\cite{mavencenter}, NPM Registry~\cite{npmregistry}, and PyPI~\cite{pypi}), the number of third-party libraries available on the Internet has grown exponentially~\cite{fse12libmigration}.
For example, from 2010 to August 2022 the number of libraries hosted on Maven Central Repository has grown from 190,446 to 9,464,023~\cite{mavenrepo}.

However, the extensive use of third-party libraries also brings the challenge of \textbf{library migration}~\cite{fse12libmigration,ese18libmigration,saner21libmigration}.
Developers often need to find alternative third-party libraries to replace the currently used ones for a variety of reasons such as sustainability failures~\cite{fse17projectfail,fse18pypi}, license restrictions~\cite{softw12license,ase14license}, absence of features~\cite{saner21libmigration}, and security/performance issues~\cite{saner21libmigration}.
For example, He \etal~\cite{fse21libmigration} analyzed the dependency changes of 17,426 open-source projects and found that 8.98\% to 28.72\% of them had undergone at least one library migration.

% describe how developer will find migration through
A prerequisite for successful library migration is finding analogical libraries (called \textbf{target libraries}) and APIs (called \textbf{target APIs}) for the currently used libraries (called \textbf{source libraries}) and APIs (called \textbf{source APIs}).
This process is known to be time-consuming, labor-intensive, and error-prone due to the large number and fast changes of third-party libraries~\cite{fse12libmigration,ese18libmigration,sevis19libevolution}. 
For example, according to Libraries.io~\cite{libariesiodata} 35,773 common Java libraries provide 15,441,057 API methods.
In this circumstance, developers often have to look for libraries and APIs with similar names as candidates and then determine whether one candidate is an analogical one by reading the lengthy API documentation~\cite{tse19apimigration}.

Many approaches have been proposed to help developers find analogical libraries~\cite{wcre12libmig,saner16libmigration,saner21libmigration,jsep14libmig,saner22libmig} and APIs~\cite{tse19apimigration,icse13apimap,wcre13funcmap,icpc19apimap,fse11apirecomd,asc20apimigration,icsme19apimig,scam15apimap}.
These approaches mainly fall into two categories, \ie evolution mining based ones and similarity calculation based ones. 
Evolution mining based approaches mine analogical library pairs~\cite{wcre12libmig,jsep14libmig,saner21libmigration} or API mappings between analogical libraries (\ie analogical API pairs)~\cite{wcre13funcmap,icsme19apimig,issrew21patternika} from the evolution history of software projects.
Similarity calculation based approaches recommend analogical libraries or APIs based on the similarity of API names, usage patterns, or text descriptions by analyzing various API documentations such as reference documentations~\cite{asc20apimigration,icpc19apimap,scam15apimap,tse19apimigration} and \SO discussions~\cite{tse21developerneed,icsme16techland,tse19apimigration,saner22libmig}.

Existing approaches heavily rely on software evolution history or API documentation to infer analogical libraries or APIs.
However, it is difficult to assume that the analyzed evolution history or API documentations have good coverage of analogical libraries or APIs, especially when the number of candidate libraries is large.
Therefore, these approaches usually cannot well support less popular libraries which are seldom involved in library migration history or online discussions.
Moreover, existing approaches for recommending analogical APIs~\cite{wcre13funcmap,icsme19apimig,issrew21patternika,tse19apimigration,asc20apimigration,icpc19apimap,scam15apimap} only support the API mapping between two specific libraries. 

In fact, it is possible to infer analogical API methods across a large number of libraries based only on the libraries themselves.
This judgment is formed based on our observations on the similarities of analogical API methods from different perspectives.
First, analogical API methods have similar API structures, including package structures, class definitions, and method declarations.
For example, some libraries for JSON processing include similar class definitions for JSON objects and JSON arrays.
Second, analogical API methods have similar functionality descriptions which may be expressed in different ways.
For example, two analogical API methods from different libraries have similar descriptions \textit{``Get the number of elements in the JSONArray''} and \textit{``Returns the number of elements in the array''}, but they use different verbs to express the same meaning.
Third, analogical API methods share similar or relevant concepts.
For example, API methods related to JSON processing often involve JSON-related concepts like JSON arrays, JSON objects, keys, and values.
Therefore, we can construct a knowledge graph capturing all these relationships and then train an embedding model for the knowledge graph. In this way, we can project the relationships from different perspectives into a unified representation space, which can realize the organic integration of knowledge from different sources~\cite{kgsurvey} to facilitate the inferring of analogical APIs.
%Inferring analogical API method needs to combine knowledge from API structures, functionality descriptions, and concepts together, but it is not easy because they are multi-source and heterogeneous.
%Constructing a knowledge graph is a good way to fuse multi-source and heterogeneous knowledge into the same dimension, by representing them as entities and relations between entities. 
%In particular, some knowledge graph embedding models have been proposed to map entities and relations into high-dimensional vector spaces, which can support inferring underlying semantic knowledge by learning from existing relationships~\cite{kgesurvey}.

In this paper, we propose an approach that can infer analogical API methods based on a large-scale analysis of third-party libraries.
The approach, called \textbf{\app} (short for \ul{\textbf{K}}nowledge \ul{\textbf{G}}raph \ul{\textbf{E}}mbedding \ul{\textbf{for}} \ul{\textbf{A}}PI \ul{\textbf{M}}igration), relies only on the libraries themselves (\eg JAR files for Java libraries) for the inference of analogical APIs.
Based on the API names, descriptions, and structures obtained from the libraries, \app constructs a unified API knowledge graph (KG for short) for a large number of third-party libraries by extracting structure knowledge of API elements (\eg package, class/interface, method, field, parameter) and functionality knowledge of API methods (\eg functionality verb and category, related concept).
\app trains a KG embedding model based on all the relation triples of the API KG.
The model provides a dense representation of the API elements in different libraries and related concepts in the form of continuous numeric vectors, which reflect the structural and conceptual relationships between API elements.
Based on the API KG and the embedding model, \app infers analogical API methods for a given API method based on the similarities of their vector representations.
Moreover, it also considers the similarities between the given API method and the neighbors of the candidate analogical API methods to re-rank the recommended API methods.

We implement \app and construct an API KG for 35,773 Java libraries. % from Libraries.io~\cite{libariesiodata}. 
The API KG contains 72,242,099 entities (including 59,155,631 API elements, 5,210,925 functionality elements, and 5,660,553 concepts) and 289,122,265 relations between them.
Then we evaluate the effectiveness and scalability of \app with the 35,773 Java libraries.
When inferring analogical API methods with given target libraries, \app achieves 47.1\%-143.0\% and 32.9\%-95.4\% improvements over the baselines in terms of MRR and Hit@10, respectively.
When inferring analogical API methods without given target libraries, \app achieves 11.6\%-80.5\%, 26.2\%-71.9\%, and 34.0\%-122.2\% improvements improvements over the baselines in terms of MRR, precision, and recall, respectively.
Moreover, \app can well scale with the increase of the number of libraries.
The resulted API KG and all the data of the evaluation can be found in our replication package~\cite{replication_package}.

%In summary, our contributions are listed as follows:
%\begin{itemize}
% 	\vspace{-1mm}
 %	\item A large-scale API KG with 72,242,099 entities and 289,122,265 relations for 35,773 Java libraries, constructed only from the implementations of libraries.
 %	\item A first-of-its-kind approach \app that infers analogical API methods across large-scale libraries using knowledge graph embedding.
%	\item An evaluation of \app for inferring analogical API methods when specifying a target library and across large-scale libraries.
 	%\item A benchmark with XXX API for evaluating analogical API inference.
%\end{itemize}


==> introduction_v2.tex <==
% Library migration is common and its basic steps
Third-party libraries have been widely used in modern software development for improving quality and productivity~\cite{softw94libreuse,ese07libreuse,fse12libmigration,ese18libmigration}. 
Meanwhile, during the rapid evolution of software systems and libraries, currently-used libraries might become unsuitable for various reasons,  such as sustainability failures~\cite{fse17projectfail,fse18pypi}, license restrictions~\cite{softw12license,ase14license}, absence of features~\cite{saner21libmigration}, and security/performance issues~\cite{saner21libmigration}; and thus developers are supposed to re-implement the same software behavior by using a different library instead of the current one. This process is known as \textit{library migration}, which has been widely observed in software evolution~\cite{}. For example, He \etal~\cite{fse21libmigration} found that 8.98\% \textasciitilde{}  28.72\% of 17,426 open-source projects undergone at least one library migration.


Given the currently-used library (called \textbf{source library}) and the API (called \textbf{source API}), the most essential part in library migration is to find an analogical library (called \textbf{target library}) and an analogical API (called \textbf{target API}), which are able to provide the same functionality as current ones. 
However, given the extremely large number and fast changes of third-party libraries and APIs~\cite{fse12libmigration,ese18libmigration,sevis19libevolution}, it is very time-consuming, labor-intensive, and error-prone for developers to find suitable target libraries and APIs. 
For example, from 2010 to August 2022, the number of libraries hosted on Maven Central Repository has grown from 190,446 to 9,464,023~\cite{mavenrepo}. In addition, Libraries.io~\cite{libariesiodata} shows that \yiling{by a time stamp?} there are 35,773 common Java libraries with 15,441,057 APIs in total. Therefore, it is a heavy burden for developers to manually look through potential libraries and APIs with similar names and read the lengthy API documentation~\cite{tse19apimigration}.

%Introduce existing api inference techniques
To reduce manual efforts in library migration, researchers have proposed many automated techniques to recommend suitable target libraries or analogical target APIs automatically. In this work, we focus on analogical API recommendation. Based on their inputs, existing analogical API recommendation techniques mainly fall into two categories, \ie evolution-mining-based ones~\cite{} and text-similarity-based ones~\cite{}.  Evolution-mining-based techniques~\cite{wcre13funcmap,icsme19apimig,issrew21patternika} take the evolution history (e.g., the code changes) as inputs and recommend analogical APIs by mining frequently-co-occurring API pairs in the existing evolution history. Textual-similarity-based ones~\cite{} mainly take the API-relevant text (e.g.,  API declarations, API functionality descriptions, or API-relevant online discussion~\cite{asc20apimigration,icpc19apimap,scam15apimap,tse19apimigration}) as input and recommend analogical APIs by calculating the textual similarity among APIs. 

% Limitation: assume that the correct target librarty is given. 
Although promising, existing approaches are designed to infer analogical APIs \textit{only between a given pair of the source library and the target library}. In other words, existing work assume that a correct target library has been already specified for API inference, which however is not always true in practice. 
In fact, choosing a suitable target library is not an easy task for developers~\cite{}. Given the limited information at hand, such a decision is often relied on domain experts or core developers~\cite{}, but it still cannot guarantee the correctness of the decision. Even if there are some automated target-library recommendation techniques, their recommendation is not always reliable in practice (e.g., Top-1 recall less than 20\%~\cite{}). Therefore, a correct target library is not always available in practice, and sometimes it might be impossible or misleading to find analogical APIs when the given target library is not a suitable choice. In summary, it is common that when developers are supposed to get rid of the current source library and its relevant APIs, they might have no clue on which target library should be used or which target library could provide analogical APIs for the current ones. 


% why existing ones cannot work on this
However, given the extremely large number of libraries and APIs, recommending analogical APIs across a large number of libraries is much more challenging that on one specific target library. Existing techniques cannot work well in this scenario due to the scalability issue. In particular, for evolution-mining-based techniques,  mining analogical APIs between one given library pair already takes non-trivial costs (e.g., \yiling{any evidence?}), and thus it is unaffordably expensive to mine API pairs between the source library and all existing libraries (e.g., XX library pairs) one by one; similarly, for text-similarity-based techniques, the online costs of calculating the similarity between the source API and target APIs in all libraries (e.g., XX API in XX libraries in total) are also very high.


The key to recommending analogical APIs across a large number of libraries is to represent and analyze similarities between so many APIs in \textit{both an effective and efficient way}. To this end, we propose \textbf{\app}, a novel approach that leverages \ul{\textbf{K}}nowledge \ul{\textbf{G}}raph \ul{\textbf{E}}mbedding \ul{\textbf{for}} analogical \ul{\textbf{A}}PI \ul{\textbf{R}}ecommendation across a large number of libraries. In particular, \app first constructs a unified API knowledge graph (KG) for a large number of third-party libraries based on their library-contained API texts; then, \app leverages graph embedding to represent nodes and edges (which indicate structural and conceptual relationships between APIs) into continuous numeric vectors; lastly, given any source API, \app recommends its analogical APIs by efficiently calculating vector similarities.  


The insights why \app could both effectively and efficiently infer analogical APIs among a large number of libraries are as follows. (1) First, \app only use the library-contained API texts (that are inherently included in libraries themselves, i.e., API declarations and functionality descriptions) as inputs. Unlike other information that are exhaustively collected from external resources (e.g., mined from evolution history~\cite{} or from Q\&A websites~\cite{}), library-contained text is prevalent and at low cost to collect, especially over a large number of libraries and APIs. %should we talk that they are also useful? 
(2) Second, using one unified API knowledge graph to represent all API-relevant text could better represent their structural and semantic information.  Although there exist other techniques that also use library-contained API texts as inputs~\cite{}, they mostly regard them as plain token sequences for similarity calculation.  However, we observe that the API-relevant texts between analogical APIs often share high structural similarity, which are very suitable for knowledge graph to represent. i) \textit{API structures} (i.e., package structures, class definitions, and method declarations) could be similar between analogical APIs. For example, some libraries for JSON processing include similar class definitions for JSON objects and JSON arrays. ii) \textit{Functionality description structures} could be similar between analogical APIs. For example,  \textit{``Get the number of elements in the JSONArray''} and \textit{``Returns the number of elements in the array''} are the functionality descriptions of two analogical API methods, and they share similar structures with different verbs to express the same meaning; iii) \textit{API concepts} are similar between analogical APIs.  For example, API  related to JSON processing often involve JSON-related concepts such as JSON arrays, JSON objects, keys, and values. \yiling{Here we need to define what is concept and what is concept in this example. Currently I cannot follow.} 
(3) Third, using graph embedding could accelerate the similarity calculation between any pair of APIs in KG. After the KG graph embedding, all APIs are represented as vectors with their relevant structural information reserved, and the similarity calculation between vectors is very fast. 
\yiling{I will revisit this paragraph after going through the approach section.}


%implementation and evaluation

We implement \app as a fully automated technique. In particular, we construct a unified API KG for 35,773 Java libraries, containing 72,242,099 entities (i.e., 59,155,631 API elements, 5,210,925 functionality elements, and 5,660,553 concepts) and 289,122,265 relations between them.\yiling{The terms of API elements, functionality elements, concepts, and relations are not explained so far. Should we use these terms, or just use the number of nodes and edges instead?}
Existing API recommendation techniques are evaluated with a given correct target library,  while this work focuses on analogical API recommendation across a large number of libraries. Therefore, to evaluate our approach, we construct a new benchmark XX. \yiling{Please talk a bit on the scale or efforts in our new benchmark. It is a contribution.} 
Our evaluation results on the new benchmark suggest that \app substantially outperforms existing analogical API recommendation techniques by achieving 11.6\%-80.5\%, 26.2\%-71.9\%, and 34.0\%-122.2\% improvements in terms of MRR, precision, and recall, respectively.
In addition, we further evaluate the scalability of \app, and the results show that \app could well scale with the increase of the number of libraries.  Moreover, we also extensively investigate the impact of different design choices in \app. 

%When inferring analogical API methods with given target libraries, \app achieves 47.1\%-143.0\% and 32.9\%-95.4\% improvements over the baselines in terms of MRR and Hit@10, respectively.

In summary, this work makes the following contributions:
\begin{itemize}
    \item \textbf{A novel approach.} We propose and implement a new analogical API recommendation approach \app by constructing and embedding a unified API knowledge graph. \app is the first technique that recommends analogical APIs across a very large number of libraries.
    
    \item \textbf{An extensive evaluation.} We extensively evaluate \app{} by comparing its effectiveness against existing techniques, investigating its scalability with different number of libraries, and studying the impact of its different design choices. 
    
    \item \textbf{A public benchmark and a large-scale API knowledge graph}. We publicly release our newly-constructed benchmark for evaluating analogical APIs across a very large number of libraries, and our constructed API knowledge graph for 35,773 Java libraries. 
\end{itemize}

All the data and code could be found in our replication package~\cite{replication_package}.



==> motivation.tex <==
Due to the resource limitation of the project running environment, Bob needs to replace currently-used API methods of \textit{gson}~\cite{gson} in the project. 
However, Bob can not find the analogical API methods directly by searching the Internet because of the lack of ready-made services and crowdsourced resources covering these APIs. 
To narrow the scope, Bob decides to find some libraries that provide features similar to \textit{gson} first.
He may locate some candidate libraries by referring to answers on technical Q\&A sites (\eg \SO), relevant blogs, or existing migration histories on GitHub.
However, none of them meet Bob's requirements.
These resources are opinion-based, with limited timeliness and coverage, tending to favor some popular libraries (\eg with many stars on GitHub) such as \textit{fastjson}~\cite{fastjson}, \textit{jackson}~\cite{jackson}.
He further searches more candidate libraries on Maven Central Repository and GitHub directly with the keywords related to the features.
But the number of candidates is usually huge, \eg a ``json'' search on Maven Central Repository returns 8,223 libraries.
In fact, a library named \textit{dsl-json}~\cite{dsl-json}, which is very small and fast, can meet Bob's needs.
However, it is not that popular, with only about 800 stars and 17 library usages on Maven Central Repository.
It is hard to find because there is very little discussion and migration history related to it.

Even if Bob finds \textit{dsl-json} luckily, he still needs to spend a lot of effort to establish the API mapping relationship.
To do this, he first determines some candidate APIs based on the names of currently-used APIs and then compares their semantics by reading their API documentation carefully.
It is difficult when Bob is unfamiliar with the library and the library has lots of APIs.
In particular, if the found library does not provide complete API mappings for all currently used APIs, he needs to repeat this process again from scratch.


In fact, we observed that even without crowdsourced resources and evolution histories of projects, the analogical relations between APIs could be inferred from the implementations of libraries.
More specifically, the analogical relations are reflected in three aspects: structures, functionalities, and concepts.

1. \textbf{Structures}. 
The API structure between analogical libraries and APIs is similar.
For example, those libraries related to JSON processing have similar classes representing JSON objects and JSON arrays, and those classes have similar methods with similar parameters and return values.

2. \textbf{Functionalities}. 
%The functionalities of methods are the key to determining whether they are analogical. 
Analogical API methods usually have the same or similar functionalities.
However, API methods with the same functionality from different libraries may express their functionalities differently~\cite{fse20funcverb}.
For example, \textit{``Get the number of elements in the JSONArray''} and \textit{``Returns the number of elements in the array''} describe the same functionality with different verbs and different concepts.

3. \textbf{Concepts}. 
APIs in analogical libraries often share many same/related concepts.
For example, many JSON-related concepts (such as JSON arrays, JSON objects, keys, values) are often mentioned in the names and descriptions of API elements for JSON processing libraries.
Moreover, the parameters, return values, and classes of analogical API methods are often related to the same concept.

This inspires us to construct a unified API KG for large-scale libraries, which includes the structure, functionality, and conceptual knowledge of API elements.
Based on this API KG, we could design an approach to infer analogical APIs across large-scale libraries. 

%, regardless of whether the library itself is popular or not.
%Based on our observations, these analogical libraries share several similarities at the API level. 

%Xie \etal~\cite{fse20funcverb} summarized some common functionality categories with functionality verbs and phrase patterns to support unified the functionalities expressed in different ways.

%It is difficult to locate analogical libraries and APIs from such a large-scale candidate, especially for some less popular features (\eg code static analysis).
\begin{comment}
	\todo{rewrite the motivation.}
	%In this chapter, we elaborate the motivation of this work in more detail.
	%Due to the large number and fast changes of third-party libraries, finding analogical libraries and APIs is not an easy task.
	%Some existing crowdsourced resources (\eg Awesome-Java\footnote{https://github.com/akullpp/awesome-java} and \SO discussion) may improve the efficiency of finding analogical libraries and APIs.
	%However, the timeliness and coverage of these crowdsourced resources are limited.
	The timeliness and coverage of existing approaches that rely on software evolution history or API documentation like Stack Overflow discussions are limited.
	Although they could help infer analogical libraries or APIs, they cannot well support less popular libraries or newly emerging ones.
	Usually, there may be multiple libraries that implement a certain feature and only a few of them are popular and used by developers very frequently.
	For example, \textit{fastjson}~\cite{fastjson}, \textit{gson}~\cite{gson}, \textit{org.json}~\cite{org.json}, \textit{jackson}~\cite{jackson}, \textit{dsl-json}~\cite{dsl-json}, and \textit{essential-json}~\cite{essential-json} are all analogical libraries related to JSON processing.
	Among them, \textit{fastjson}, \textit{gson}, \textit{org.json}, and \textit{jackson} are very popular, indicated by .
	While \textit{dsl-json} is less popular w and \textit{essential-json} is a new library created at 2019.
	Existing approaches tend to favor popular libraries, and it is difficult to cover less popular libraries, not to mention those newly emerging ones.
	However, in some cases, the less popular or new libraries could be more suitable for developers than popular libraries because of their special characteristics.
	For example, \textit{dsl-json} and \textit{essential-json} are small and fast, which is useful when the computation resources are limited.
	Moreover, libraries that implement a certain feature only account for a small part of the total number of third-party libraries. 
	It is difficult to locate analogical libraries and APIs from such a large-scale candidate, especially for some less popular features (\eg code static analysis).
	Furthermore, at the API level, even the APIs of popular libraries are not all popular, and only a small part of APIs have rich evolution history and documentation.
	Therefore, we need a way to find analogical APIs across large-scale third-party libraries.
	%Based on our observations, the analogical APIs from different libraries have high similarity in their structures, functionalities, and concept associations, which are indicated by the libraries themselves.
\end{comment}



%However, APIs with the same functionality from different libraries may express their functionalities differently~\cite{fse20funcverb}.
%For example, \textit{``return the length''} and \textit{``get the length''} describe the same functionality with different verbs. 
%be described with different functionality verbs and phrase patterns~\cite{fse20funcverb}. 
%For example, \textit{``return length''} and \textit{``get length''} describe the same functionality. 


%Figure~\ref{fig:kgexample} shows a pair of analogical API methods (\ie \textit{org.json.JSONArray.length()} and \textit{com.google.gson.JsonArray.size()}) from two analogical libraries (\ie\textit{org.json}~\cite{org.json} and \textit{com.google.code.gson:gson}~\cite{gson}), respectively, with their relations in an API knowledge graph. 
%As shown in Figure~\ref{fig:kgexample}, these two methods have rich associations in the API KG through API structures (\eg same type return value), functionalities (\eg similar functionalities), and concepts (\eg related to json array, element number), implying an analogical relationship between them.
%The information in the API knowledge graph can be obtained from the source code of libraries by analyzing the API structure, names, and description text from comments.

%In this situation, there are a lot of library migration history and online discussions involving popular ones, and very little about the less popular one.


%Existing approaches heavily rely on software evolution history or API documentation to infer analogical libraries or APIs.
%However, it is difficult to assume that the analyzed evolution history or API documentations have good coverage of analogical libraries or APIs, especially when the number of candidate libraries is large.
%Therefore, these approaches usually cannot well support less popular libraries which are seldom involved in library migration history and online discussions.
%Moreover, existing approaches for recommending analogical APIs~\cite{wcre13funcmap,icsme19apimig,issrew21patternika,tse19apimigration,asc20apimigration,icpc19apimap,scam15apimap} only support the API mapping between two specific libraries. 

%Existing approaches that rely on software evolution history and online discussions could help infer analogical libraries or APIs.
%However, they also have co 



%There are a lot of library migration history and online discussions involving popular ones, and very little about the less popular one.
%Therefore, existing approaches that rely on software evaluation history and online discussions tend to favor popular libraries, and it is difficult to cover less popular libraries like dsl-json.
%However, \textit{dsl-json} has some features, such as the smallest size, safe code, and fast speed, which is useful for developers with special needs.

%Existing approaches for recommending analogical APIs~\cite{wcre13funcmap,icsme19apimig,issrew21patternika,tse19apimigration,asc20apimigration,icpc19apimap,scam15apimap} only support the API mapping between two specific libraries. 

%Therefore, these approaches usually cannot well support less popular libraries which are seldom involved in library migration history and online discussions.
%Moreover, existing approaches for recommending analogical APIs~\cite{wcre13funcmap,icsme19apimig,issrew21patternika,tse19apimigration,asc20apimigration,icpc19apimap,scam15apimap} only support the API mapping between two specific libraries. 

%Due to the large number and fast changes of third-party libraries~
%Finding analogical libraries and APIs is not a easy task, 
%要点：
%1）实现某类功能的lib有很多个，有一些不是那么热门但也有自身的特点，但同时在大量的候选库中仍然是很少的一部分。
%注：目前方法部分的例子是两个热门库，体现不出我们方法的特点
%2）这些可类比的lib在API层面上存在多个方面的相似性，每个方面作为一个要点进行介绍并举例说明。注意例子要跨越多个lib，而不是总在两个lib之间。同时强调这些信息都是从lib本身就可以获取的。

%Some existing crowdsourced resources (\eg Awesome-Java\footnote{https://github.com/akullpp/awesome-java} and \SO) may improve the efficiency of finding analogical libraries and APIs.
\begin{comment}
A prerequisite for successful library migration is finding analogical libraries (called \textbf{target libraries}) and APIs (called \textbf{target APIs}) for the currently used libraries (called \textbf{source libraries}) and APIs (called \textbf{source APIs}).
This process is known to be time-consuming, labor-intensive, and error-prone due to the large number and fast changes of third-party libraries~\cite{fse12libmigration,ese18libmigration,sevis19libevolution}. 
For example, according to Libraries.io~\cite{libariesiodata} \update{35,773} common Java libraries provide \update{15,441,057} API methods.
In this circumstance, developers often have to look for libraries and APIs with similar names as candidates and then determine whether one candidate is an analogical one by reading the lengthy API documentations~\cite{tse19apimigration}.
Many approaches have been proposed to help developers find analogical libraries~\cite{wcre12libmig,saner16libmigration,saner21libmigration,jsep14libmig,saner22libmig} and APIs~\cite{tse19apimigration,icse13apimap,wcre13funcmap,icpc19apimap,fse11apirecomd,asc20apimigration,icsme19apimig,scam15apimap}.
These approaches mainly fall into two categories, \ie evolution mining based ones and similarity calculation based ones. 
Evolution mining based approaches mine analogical library pairs~\cite{wcre12libmig,jsep14libmig,saner21libmigration} or API mappings between analogical libraries (\ie analogical API pairs)~\cite{wcre13funcmap,icsme19apimig,issrew21patternika} from the evolution history of software projects.
Similarity calculation based approaches recommend analogical libraries or APIs based on the similarity of API names, usage patterns, or text descriptions by analyzing various API documentations such as reference documentations~\cite{asc20apimigration,icpc19apimap,scam15apimap,tse19apimigration} and \SO discussions~\cite{tse21developerneed,icsme16techland,tse19apimigration,saner22libmig}.

Existing approaches heavily rely on software evolution history or API documentation to infer analogical libraries or APIs.
However, it is difficult to assume that the analyzed evolution history or API documentations have good coverage of analogical libraries or APIs, especially when the number of candidate libraries is large.
Therefore, these approaches usually cannot well support less popular libraries which are seldom involved in library migration history and online discussions.
Moreover, existing approaches for recommending analogical APIs~\cite{wcre13funcmap,icsme19apimig,issrew21patternika,tse19apimigration,asc20apimigration,icpc19apimap,scam15apimap} only support the API mapping between two specific libraries. 


\end{comment}



%The rationale is that historical migration practices can provide reference and guidance for developers to make new ones~\cite{saner21libmigration}.
%Similarity calculation based approaches recommend analogical libraries~\cite{saner22libmig,saner16libmigration} or APIs~\cite{fse11apirecomd,icpc19apimap,tse19apimigration,asc20apimigration} based on the similarity of API names, usage patterns, or text descriptions by analyzing various API documentations such as reference documentations and \SO discussions~\cite{tse21developerneed,icsme16techland,tse19apimigration,saner22libmig}.

%Some existing crowdsourced resources (\eg Awesome-Java\footnote{https://github.com/akullpp/awesome-java} and \SO) may improve the efficiency of finding analogical libraries and APIs.
%API name similarity~\cite{tse19apimigration,asc20apimigration}, 
%API usage pattern similarity~\cite{tse19apimigration}, 
%documentation similarity~\cite{tse19apimigration,asc20apimigration,icpc19apimap}.


%The model can map the entities and relations of the KG to high-dimensional dense vectors which encode the structure information of the KG.
%Thus we could train a knowledge graph embedding are trained based on the relation triples of API KG for each entities and relations, which captures the structural and semantic relationships between APIs.
%To tackle these limitations, our idea is to build a unified API KG for large-scale third-party libraries based on their source code, and then infer analogical APIs across libraries by using the knowledge graph embedding encoding the knowledge of the knowledge graph.


%require that the target library of the migration is known.

%specifying the source-target library pair as input.
%More importantly, some unpopular/newly emerging libraries/APIs may lack project code or high-quality documentation, which has a great impact on the actual performance of those techniques.
%Collecting, processing, and updating the required data is not a simple task due to the numerous and constantly emerging libraries.
%More importantly, some unpopular/newly emerging libraries/APIs may lack project code or high-quality documentation, which has a great impact on the actual performance of those techniques.

\begin{comment}
	Existing approaches heavily rely on software evolution history or API documentations to infer analogical libraries or APIs.
	However, it is difficult to assume that the analyzed evolution history or API documentations have a good coverage of analogical libraries or APIs, especially when the number of candidate libraries is large.
	Therefore, these approaches usually cannot well support less popular libraries which are seldom involved in library migration history and online discussions.
	Moreover, existing approaches for recommending analogical APIs~\cite{??, ??} only support the API mapping between two specific libraries. 
\end{comment}



%However, APIs with the same functionality from different libraries may express their functionalities differently~\cite{fse20funcverb}.
%For example, \textit{``return the length''} and \textit{``get the length''} describe the same functionality with different verbs. 
%be described with different functionality verbs and phrase patterns~\cite{fse20funcverb}. 

%The functionalities of methods are the key to determining whether they are analogical. 
%However, APIs with the same functionality from different libraries may express their functionalities differently~\cite{fse20funcverb}.
%For example, \textit{``return the length''} and \textit{``get the length''} describe the same functionality with different verbs. 
%be described with different functionality verbs and phrase patterns~\cite{fse20funcverb}. 
%For example, \textit{``return length''} and \textit{``get length''} describe the same functionality. 
%Xie \etal~\cite{fse20funcverb} summarized some common functionality categories with functionality verbs and phrase patterns to support unified the functionalities expressed in different ways.

%For example, analogical API methods in the API KG may have similar API structure information (\eg their API libraries have similar organization structures) or have many shared neighbors (\eg functionalities, concepts).

%Designers of different third-party libraries may use similar concepts with subtle differences in the names and descriptions of API elements, such as ``json array'' and ``jsonarray''. 

%Leveraging API documentation to map APIs has been explored by previous studies, and recently, code-based learning approaches have become the mainstream approach and shown better results. 

%However, learning approaches often require a large amount of training data (e.g., projects implemented using multiple languages or API mapping datasets), which are not widely available. In contrast, API documentation is usually available, but we have observed that much information in API documentation has been underexploited. Therefore, we develop a deep-dive approach to extensively explore API documentation to create improved API mapping methods. Our documentation exploration approach involves analyzing the functional description of APIs, and also considers the parameters and return values. The results of this analysis can be used to generate not only one-to-one API mapping, but also compatible API sequences, thereby enabling one-to-many API mapping. In addition, parameter-mapping relationships, which have often been ignored in previous approaches, can be produced. We apply this approach to map APIs from Java to Swift, and the experimental results indicate that our deep-dive analysis of API documentation leads to API mapping results that are superior to those generated by existing approaches

%save both time and resources and reduce redundancy by taking advantage of existing quality implementations.

==> related_worl_bak.tex <==
We summarize and compare related work from three aspects: analogical library recommendation, analogical API recommendation, and knowledge graph in software engineering.

\subsection{Analogical Library Recommendation}
Research into analogical library recommendations has a long history.
Most of the previous work focused on mining the evolution history of projects~\cite{wcre12libmig,jsep14libmig,icsme19apimig,saner21libmigration}, \ie evolution mining based methods.
The rationale is that historical migration records could provide reference and guidance for developers when they make migration decisions.
For example, Teyton \etal \cite{wcre12libmig} propose an approach to mine library migration rules from the dependency changes of projects. % and build a library migration graph with relations between analogical libraries.   
%Recently, He \etal \cite{saner21libmigration} proposed a library migration recommendation method that combines mining and ranking steps. 
%They first generate possible library migration candidates by pre-mining the dependency change records of large-scale software projects and then rank the candidates by combining multiple metrics such as the number of supporting migration records and commit messages.
%These evolution mining based methods are suitable for popular libraries with migration histories, but fail to support newly emerging or less popular libraries with no or little relevant migration histories.
However, these evolution mining based methods cannot well support less popular libraries which are seldom involved in library migration history.
%These evolution mining based methods are suitable for popular libraries with migration histories, but fail to support newly emerging or less popular libraries with no or little relevant migration histories.

Another line of research use similarity calculation based approaches to recommend analogical libraries~\cite{saner16libmigration,saner22libmig,ese19libmig,ase16simtech,icsme16techland}.
% by considering the crowdsourced knowledge from \SO~\cite{saner16libmigration,saner22libmig,ese19libmig,ase16simtech,icsme16techland}.
%For example, Chen \etal \cite{saner16libmigration} recommend analogical libraries by combining word embeddings and domain knowledge trained/extracted from \SO tags. 
For example, Nafi \etal \cite{saner22libmig} propose a tool named XLibRec for recommending analogical libraries across different programming languages, which is based on the library-related discussions from \SO and library documentation from Libraries.io.
%They generate three different vector representations for each library based on the library-related question titles, answer body, and descriptions and then calculate a weight-based cosine similarity between the vector representations of libraries to recommend libraries.
However, these approaches still do not work well for libraries that are rarely discussed on \SO.

Unlike the above approaches, we focus on inferring analogical API methods, which are more fine-grained and do not require evolution history and online discussions. 
%Further, our approach does not rely on evolution history and \SO involving libraries, but only on their implementations.

\subsection{Analogical API Recommendation}
Similar to analogical library recommendation, approaches proposed for analogical API recommendation are also divided into evolution mining based ones~\cite{wcre13funcmap,icsme19apimig,issrew21patternika} and similarity calculation based ones~\cite{asc20apimigration,icpc19apimap,scam15apimap,tse19apimigration,tse21developerneed,saner22libmig}. 

Evolution mining based ones focus on mining API mappings from existing migrations.
For example, Teyton \etal \cite{wcre13funcmap} find API mappings by analyzing their co-occurring frequencies in existing migrations. 
%Similarly, Blech \etal \cite{issrew21patternika} propose Patternika, a pattern-mining-based method to mine API migration patterns from historical library migration instances via static code differencing technique.
Similarity calculation based approaches recommend analogical APIs based on the similarity of API names, usage patterns, or text descriptions by analyzing various API documentations such as reference documentations~\cite{asc20apimigration,icpc19apimap,scam15apimap,tse19apimigration} and \SO~discussions~\cite{tse21developerneed,saner22libmig}.
%For example, Pandita \etal \cite{scam15apimap} adopt text mining to identify likely API mappings based on the textual similarity of API names and documents. 
For example, Alrubaye \etal used information retrieval techniques~\cite{icpc19apimap} and machine learning models~\cite{asc20apimigration} to mine similar APIs, which both use similarities between method signatures and textual documentation as inputs.
%The above approaches all rely on the traditional statistic-based text similarity method, namely TF-IDF.
Recently, learning-based semantic vector similarity has become popular.
For example, Chen \etal \cite{saner16libmigration} used an unsupervised deep learning based approach to represent API usage patterns and API descriptions into a vector space respectively and infer likely analogical API mappings between libraries by combining API similarity in different vector spaces.

Existing approaches heavily rely on software evolution history or API documentation to infer analogical APIs, with limited coverage of analogical APIs from a large number of libraries. 
Moreover, the above approaches for recommending analogical APIs only support the API mapping between two specific libraries. 
On the contrary, our approach can support inferring analogical API methods without given target libraries based on the unified API knowledge graph. 

%Some other works focus on cross-language API mapping by using API reference documentation based on similarity~\cite{icpc20apimigration} or learning on large-scale software project~\cite{icse16deepapi}.
%Some other works focus on cross-language API mapping (\eg JDK APIs to Swift APIs) by using API reference documentation based on similarity~\cite{icpc20apimigration} or learning on large-scale software project~\cite{icse16deepapi}.
%These approaches can be treated as recommending analogical APIs in a specified target library as well, which require large amount of project code or high-quality documentation as well. 
%Therefore, their approaches can not be adopted in large-scale third-party libraries either.

%For example, Zhang \etal \cite{icpc20apimigration} mine Java-to-Swift API mapping based on the analysis of API documentation, which considering the functional description, parameters and return values. 

%Alrubaye \etal \cite{asc20apimigration} proposed RAPIM, a machine learning based method that recommend API method mappings between two given libraries. RAPIM relies on some manually selected use similarity between method signatures and textual documentation as inputs.

%Evolution mining based approaches mine analogical library pairs~ or API mappings between analogical libraries (\ie analogical API pairs)~\cite{wcre13funcmap,icsme19apimig,issrew21patternika} from the evolution history of software projects.
%
%Therefore, these approaches usually cannot well support less popular libraries which are seldom involved in library migration history and online discussions.
%Moreover, existing approaches for recommending analogical APIs~\cite{wcre13funcmap,icsme19apimig,issrew21patternika,tse19apimigration,asc20apimigration,icpc19apimap,scam15apimap} only support the API mapping between two specific libraries. 
%Evolution mining based approaches mine analogical library pairs~\cite{wcre12libmig,jsep14libmig,saner21libmigration} or API mappings between analogical libraries (\ie analogical API pairs)~\cite{wcre13funcmap,icsme19apimig,issrew21patternika} from the evolution history of software projects.

%Some studies proposed methods for mining API mappings of two given similar libraries~\cite{fse11apirecomd,asc20apimigration,saner16libmigration,wcre13funcmap,icpc19apimap,icse13apimap}.
%Gokhale \etal \cite{icse13apimap} mine the the execution traces of program to find similar APIs. 
%Zheng  \etal \cite{fse11apirecomd} mine alternative APIs from developer shared knowledge in forums or blog posts. 
%Collie \etal \cite{ase20m3apimap} identified migration mappings by modeling and synthesizing library API behavior without prior knowledge. \todo{re-write the related work.}
%Zheng \etal \cite{fse11crosslibapirecom} proposed a cross-library recommendation tool based on Web queries using search engines such as Google. \todo{refine}
%icsme19apimig
\subsection{Knowledge Graph in Software Engineering}
Recently, researchers in the software engineering domain have constructed knowledge graphs for different kinds of knowledge and purposes such as API caveats~\cite{icsme2018apicaveat}, domain terminology~\cite{fse2019glossary}, API concepts and descriptive knowledge~\cite{fse19apisummary}, and programming tasks~\cite{fse22taskkg}.
Different from their work, \app is the first one to apply the API knowledge graph for inferring analogical API methods. 
Among them, Liu \etal \cite{ase20apicomp} also built an API knowledge graph.
However, our API knowledge graph is very different from theirs on the scales and goals.
They only built an API knowledge graph for JDK and Android SDK and their goal is to support generating an API comparison table for a pair of APIs.
%On the contrary, we build an API knowledge graph for large-scale Java libraries and use it to infer analogical API methods.


%Different from their work, \app is the first one to apply the API knowledge graph for analogical API method inferring through knowledge graph embedding. scale, structure data source, usage, and purpose. from API documents. Their goal, however, is to generate a comparison table for comparable APIs of the same library to illustrate their differences. 

\begin{comment}
	\subsection{Others}
	A prerequisite for successful library migration is finding analogical libraries (called \textbf{target libraries}) and APIs (called \textbf{target APIs}) for the currently used libraries (called \textbf{source libraries}) and APIs (called \textbf{source APIs}).
	This process is known to be time-consuming, labor-intensive, and error-prone due to the large number and fast changes of third-party libraries~\cite{fse12libmigration,ese18libmigration,sevis19libevolution}. 
	For example, according to Libraries.io~\cite{libariesiodata} \update{35,773} common Java libraries provide \update{15,441,057} API methods.
	In this circumstance, developers often have to look for libraries and APIs with similar names as candidates and then determine whether one candidate is an analogical one by reading the lengthy API documentations~\cite{tse19apimigration}.
	
	Many approaches have been proposed to help developers find analogical libraries~\cite{wcre12libmig,saner16libmigration,saner21libmigration,jsep14libmig,saner22libmig} and APIs~\cite{tse19apimigration,icse13apimap,wcre13funcmap,icpc19apimap,fse11apirecomd,asc20apimigration,icsme19apimig,scam15apimap}.
	These approaches mainly fall into two categories, \ie evolution mining based ones and similarity calculation based ones. 
	Evolution mining based approaches mine analogical library pairs~\cite{wcre12libmig,jsep14libmig,saner21libmigration} or API mappings between analogical libraries (\ie analogical API pairs)~\cite{wcre13funcmap,icsme19apimig,issrew21patternika} from the evolution history of software projects.
	Similarity calculation based approaches recommend analogical libraries or APIs based on the similarity of API names, usage patterns, or text descriptions by analyzing various API documentations such as reference documentations~\cite{asc20apimigration,icpc19apimap,scam15apimap,tse19apimigration} and \SO discussions~\cite{tse21developerneed,icsme16techland,tse19apimigration,saner22libmig}.
	
	Existing approaches heavily rely on software evolution history or API documentation to infer analogical libraries or APIs.
	However, it is difficult to assume that the analyzed evolution history or API documentations have good coverage of analogical libraries or APIs, especially when the number of candidate libraries is large.
	Therefore, these approaches usually cannot well support less popular libraries which are seldom involved in library migration history and online discussions.
	Moreover, existing approaches for recommending analogical APIs~\cite{wcre13funcmap,icsme19apimig,issrew21patternika,tse19apimigration,asc20apimigration,icpc19apimap,scam15apimap} only support the API mapping between two specific libraries. 
	
	Lu \etal \cite{ksem17apimap} and Gu \etal \cite{ijcai17deepapm} infer similar APIs across different programming languages from API documents. 
	% Documentation based apporach 
	% Code based apporach
	% Documentation 
	
	A previous study by Liu \etal \cite{ase20apicomp} shows that the API knowledge graph (KG for short) can provide knowledge explanations for analogical API pairs of a single library~\cite{ase20apicomp}.
	They found that analogical APIs are close in the API KG by sharing many neighbors and relationships, \eg concepts, and functionalities.
	Extending their ideas, we can build a unified API KG for large-scale third-party libraries to support inferring analogical APIs across libraries. 
	%, which includes knowledge of with API structural knowledge, functionalities, and conceptual knowledge
	%However, the method of Liu \etal requires high-quality API reference documentation as input for API KG construction. 
	In order to improve the coverage of the API KG and reduce the construction cost, the input should be as simple and easy to obtain as possible, \eg, only the source code of third-party libraries.
	Furthermore, the API KG is discrete, which is difficult to directly use for inferring analogical APIs.
	Knowledge graph embedding is a task of learning a low-dimensional representation of entities and relations in a knowledge graph while preserving their semantic meaning~\cite{tkde17kgesurvey}.
	Through knowledge graph embedding, analogical APIs with similar structures, functionalities, and conceptual associations in the API KG are close to each other in the vector space (see Figure~\ref{fig:kg_emb_example}), which enables more efficient support for analogical API inference.
\end{comment}


==> rq2_bak.tex <==
We compare \app with baselines on inferring analogical API methods for randomly selected API methods without given target libraries.
%We can compare the performance of \app and the baselines for inferring analogical API methods across large-scale libraries. 
%To compare with them more fairly, we also restrict \app to only infer analogical API methods on the target library.
%BM25-based baseline We compare \app with baselines from previous work and a variant of \app, \ie RAPIM, D2APIMap, and \app-Ret.
\subsubsection{Baselines}
The baselines used in RQ1 (\ie RAPIM and D2APIMap) do not support inferring analogical API methods without given target libraries.
To this end, we first create a simple baseline by using BM25~\cite{bm25}.
BM25 is an information retrieval approach used by search engines to estimate the relevance of documents to a given search query.
We construct the document for each API method in the API KG by combining its method name and description.
We compute the BM25 score between the query API method and the documents for all API methods and return the top-$n$ API methods with the highest scores.
To improve performance of BM25, we clean the documents and the query API according to previous work~\cite{icpc20apimigration}, including stop word removal, camel case splition, and lemmatization. 
We implement the BM25 baseline by using Elasticsearch~\cite{elasticsearch}.
Then, we combine BM25 with RAPIM and D2APIMap respectively to create two baselines BM25+RAPIM and BM25+D2APIMap.
They use BM25 to obtain the top-$n$ 100 results as candidates and then re-rank candidate based on RAPIM or D2APIMap.
We set $n$ to be 100, which is the same as the retrieval step in \app.

\subsubsection{Protocol}
The benchmark in RQ1 is not suitable for evaluating the inferring analogical API methods without given target libraries.
Therefore, we manually select 9 pairs of analogical libraries (\ie 18 libraries) based on previous work~\cite{tse19apimigration} and our expert knowledge, covering popular libraries (\eg \textit{gson}~\cite{gson}) and less popular libraries (\eg \textit{dsl-json}~\cite{dsl-json} and \textit{dom4j}~\cite{dom4j}).
For each of these 18 libraries, we randomly select 15 API methods in the library as the query API methods for evaluation, leading to 270 query API methods.
For each query API method, we retrieve the top-10 results returned by \app and the baselines (\ie BM25, BM25+RAPIM, and BM25+D2APIMap).
Note that we remove the API methods with the exact same name as the query API method from the results. 
Because some libraries may completely include other libraries in their implementations.
We merge the search results for the same query API method and remove the duplicate results.
Then we invite 6 participants (MS students with more than three years of Java development experience each) to assess whether the returned API methods are analogical to the query API method. 
All results retrieved for a query API method are assessed by the same two participants independently.
Participants are asked to read the API reference documentation of query API method and returned API methods to make the judgment.
All retrieval results for the same query API method are shuffled before assessment and participants do not know which approach retrieve the result. 
If the assessment of two annotators for the same retrieved result was inconsistent, a third annotator is assigned to produce an additional judgment, and the final annotation is determined based on the majority.
As a result, the agreement between the judgments is substantial (\ie Cohen's Kappa coefficient~\cite{kappa} of 0.666).
Based on the ground truths obtained after annotation, we could compare \app and the baselines in terms of MRR, precision, and recall.
Precision is the fraction of analogical API methods among the returned results, while recall is the fraction of analogical API methods that are retrieved. 
\subsubsection{Results}
\begin{table}[]
	%\scriptsize
	\centering
	%\vspace{-7mm}
	\caption{Performance Comparison between \app and Baselines without Given Target Libraries}
	\label{tab:rq1:effiveness:cross_lib}
	\footnotesize
	\vspace{-3mm}
	\begin{tabular}{|c|c|c|c|}
		\hline
		Approach    & MRR & Precision & Recall  \\ \hline
		BM25        &  0.557   &  0.318    &   0.325           \\ \hline
		BM25+RAPIM  & 0.381  &  0.271   &   0.216       \\ \hline
		BM25+D2APIMap  & 0.616    &  0.369   &   0.358         \\ \hline
		\app   &  \textbf{0.688}  &   \textbf{0.466}  & \textbf{0.480}     \\ \hline
	\end{tabular}
	\vspace{-5mm}
\end{table}
The evaluation results are shown in Table~\ref{tab:rq1:effiveness:cross_lib}.
Overall, \app outperforms all the baselines on all metrics by achieving 11.6\%-80.5\%, 26.2\%-71.9\%, and 34.0\%-122.2\% improvements over the baselines in terms of MRR, precision, and recall, respectively.
Compared with the best baselines (\ie BM25+D2APIMap), the improvements in precision and recall are more significant (\ie 26.2\% and 34.0\%, respectively) than MRR (\ie 11.6\%).
After analysis, we find that in the case of large number of libraries and APIs, it is more likely that there are analogical API methods with very close or even identical names to the query API method.
These API methods are easily retrieved by text similarity based methods like BM25 with high rankings, resulting in high MRR for the baselines.
%However, such easy cases are only a few.
However, these API methods are easy cases and \app can discover more analogical API methods accurately, which is more meaningful for developers.
%by providing more candidates.
Moreover, \app can achieve a more significant performance difference than the baselines for less popular libraries. 
For example, the MRR, precision, and recall of \app on \textit{dsl-json}~\cite{dsl-json} (with only 817 stars on GitHub) are 0.542, 0.327, 0.562, respectively; while these metrics of BM25+D2APIMap on the same library are only 0.206, 0.080, and 0.171, respectively.
\subsubsection{Summary}
%In summary, 
\app outperforms three baselines for inferring analogical API methods without given target libraries.
%These results suggest that \app can effectively support inferring analogical API methods even without specifying a target library.

==> rq3_bak.tex <==
We conduct some experiments to explore the impact of some key factors on \app, \ie KG embedding models, knowledge types, and similarity types and weights.
To conduct various factor-related experiments more conveniently, we construct a small-scale API KG whose input is the all libraries involved in the benchmark of RQ1, \ie 16 libraries.
\subsubsection{Impact of KG Embedding Models}
We train different KG embedding models on the small-scale API KG to explore which ones are more suitable for inferring analogical API methods.
We try ComplEx and two other popular KG embedding models, TransE~\cite{transE} and DistMult~\cite{DistMult}.
We evaluate the performance of KG embedding models by evaluating the \app-Ret baseline on the benchmark for inferring analogical API methods with given target libraries (see Section~\ref{sec:rq1}) with different KG embedding models.
\app-Ret retrieves analogical API methods based on the KG embedding similarity between methods, whose performance can well reflect how much the KG embedding model learns the semantics of API methods.
We compare different KG embedding models on the top 100 results.
The results are shown in Table~\ref{tab:kge}.
The ComplEx model achieves the best performance on all metrics, therefore ComplEx is used in our implementations.
\begin{table}[]
	%\scriptsize
	\centering
	%\vspace{-4mm}
	\caption{Impact of Different Knowledge Graph Embedding Models}
	\label{tab:kge}
	\footnotesize
	\vspace{-1mm}
	\textbf{}	\begin{tabular}{|p{2cm}<{\centering}|c|c|c|p{0.7cm}<{\centering}|p{0.8cm}<{\centering}|}
		\hline
		Method     & MRR & Hit@1 & Hit@3 & Hit@5 & Hit@10\\ \hline
		%TransE+Softmax     &   0.235  &    0.139   &   0.244   &  0.335     &   0.448     \\ \hline
		TransE    &  0.284  &  0.174    &  0.312    &  0.396   &   0.518     \\ \hline
		%DistMult+Softmax   &  0.289   &    \textbf{0.183}  &   0.324    &   0.404    &    0.507     \\ \hline
		DistMult  &  0.288   &     0.180  &  \textbf{0.331}   & 0.400     &  0.494      \\ \hline
		%ComplEx+Softmax    &  0.269   &   0.161   & 0.294      & 0.389     & 0.509      \\ \hline
		ComplEx   &  \textbf{0.293}   &   \textbf{0.183}  & 0.324    &\textbf{0.422}   &   \textbf{0.524}   \\ \hline
		
		%TransE+Softmax     &   0.235  &    0.139   &   0.244   &  0.335     &   0.448     \\ \hline
		%TransE+Logistic    &  0.284  &  0.174    &  0.312    &  0.396   &   0.518     \\ \hline
		%DistMult+Softmax   &  0.289   &    \textbf{0.183}  &   0.324    &   0.404    &    0.507     \\ \hline
		%DistMult+Logistic  &  0.288   &     0.180  &  \textbf{0.331}   & 0.400     &  0.494      \\ \hline
		%ComplEx+Softmax    &  0.269   &   0.161   & 0.294      & 0.389     & 0.509      \\ \hline
		%ComplEx+Logistic   &  \textbf{0.293}   &   \textbf{0.183}  & 0.324    &\textbf{0.422}   &   \textbf{0.524}   \\ \hline
	\end{tabular}
\vspace{-3mm}
\end{table}

\subsubsection{Impact of Knowledge Types in the API Knowledge Graph}
To evaluate the impact of different types of knowledge in the API KG, we train different KG embedding models based on a subset of relation triples in the small-scale API KG.
We try three situations: only structural relation triples (denoted as \textit{Structure}), all relation triples except functionality-related relations (denoted as \textit{Functionality*}), and all relation triples except conceptual relations (denoted as \textit{Concept*}).
Then we evaluate different KG embedding models based on \app-Ret and the benchmark as well.
The results are shown in Table~\ref{tab:knowledge_type}.
Both functionality and conceptual contribute positively to analogical API method inferring, while conceptual knowledge has a greater impact than functionality knowledge.

%ComplEx model achieves the best performance on all metrics, therefore ComplEx is used our implementations.

\begin{table}[]
	%\scriptsize
	\centering
	\vspace{-1mm}
	\caption{Impact of Different Knowledge Types}
	\label{tab:knowledge_type}
	\footnotesize
	\vspace{-3mm}
	\begin{tabular}{|c|c|c|c|p{0.6cm}<{\centering}|p{0.8cm}<{\centering}|}
		\hline
		Knowledge Type     & MRR & Hit@1 & Hit@3 & Hit@5 & Hit@10  \\ \hline
		Structure         &  0.154   &  0.070     &   0.169    &   0.233    &     0.331          \\ \hline
		Functionality*  & 0.282    &  \textbf{0.185}   &   0.309     &  0.385     &       0.489        \\ \hline
		Concept*  &   0.237  &    0.150   &   0.259    &   0.335    &      0.422      \\ \hline
		All   &  \textbf{0.293}   &   0.183  & \textbf{0.324}    &\textbf{0.422}   &   \textbf{0.524}   \\ \hline
	\end{tabular}
	\vspace{-5mm}
\end{table}

\subsubsection{Impact of Similarity Types and Similarity Weights}
\begin{figure}
	\centering
	%\vspace{-7mm}
	\includegraphics[width=0.65\columnwidth]{images/number_fold}
	\vspace{-5mm}
	\caption{Impact of the Number of Data Used for Tuning Weights}
	\vspace{-8mm}
	\label{fig:fold_num}
\end{figure}
To obtain good weights for the similarities (\ie $W_{m}$, $W_{func}$, $W_{obj}$, $W_{it}$, $W_{iv}$, $W_{ot}$, and $W_{neig}$) used in the re-ranking step (see Section~\ref{sec:candidate_rerank}), we tune them on the small-scale API KG based on the benchmark.
In order to prevent overfitting, we do not directly tune the weights on the large-scale API KG.
We use Beam search~\cite{beamsearch} to tune all weights one by one with a step size of 0.05 and a beam number of 4.
The combination of weights with the best MRR metric is retained. 
As a result, the best weights are:  $W_{m}=0.05$, $W_{func}=0.95$, $W_{obj}=0.8$, $W_{it}=0.25$, $W_{iv}=0.05$, $W_{ot}=0.05$, and $W_{neig}=0.95$.
In order to explore the impact of tuning data on our performance, we randomly divide the benchmark data into 10 folds and then use a different number of folds to tune the weights in turn.
Figure~\ref{fig:fold_num} shows experimental results in RQ1 (\ie inferring analogical API methods with given target libraries) under weights tuned with different folds of data, which is on the large-scale API KG and its KG embedding model.
We can see that the final metric increases as more data are used to tune the weights,
However, the differences between the different metrics are not large, indicating that tuning the weights with fewer data can already achieve acceptable performance.
Note that our weight tuning is based on a small-scale API KG, while the final RQ1 experiments are based on a large-scale API KG.
This proves that our weights can generalize even on different API KGs.
We try to remove each of the similarities for evaluation in large-scale API KG (\ie set the weight of the similarity to 0).
Table~\ref{tab:rerank_sim} shows the evaluation results, where $Sim_{t}*$ represents removing the similarity $Sim{t}$.
We can see that after removing each similarity, the performance of \app decreases. 
Among them, removing functionality similarity $Sim_{func}$ has the greatest impact, with MRR dropping by 22.9\%.
This reflects the importance of the functionality knowledge for analogical API method inferring.
After removing $Sim_{neig}$, MRR increases and Hit@10 decreases, indicating that considering the overall similarity of neighbors brings some noise while improving recall.
%First, we obtain the top-100 candidate API methods for all query API methods in the benchmark.
%Then we try different weight for the re-ranking, and retain the weight combination with the best MRR metric.
\begin{comment}
	In order to evaluate the impact of different types of knowledge in the API KG, we trained different KG embedding models based on subset of relation triples in the small-scale API KG, including only structural relation triples (denoted as \textit{Structure}), all relation triples except functionality-related relations (denoted as \textit{Functionality*}), and all relation triples except conceptual relations (denoted as \textit{Concept*}).
	Then we evaluate different KG embedding model based on \app-Ret and the benchmark as well.
	The results are shown in Table~\ref{tab:knowledge_type}.
	Both functionality and conceptual knowledge contribute positively to analogical API method inferring, with conceptual knowledge having a greater impact than functionality knowledge.
\end{comment}

\subsubsection{Summary}
The KG embedding model, knowledge types, and similarity types and weights have a large impact on the performance of \app.

\begin{table}[]
		%\scriptsize
		\centering
		%\vspace{-7mm}
		\caption{Contribution of Different Similarities in the Re-ranking Step}
		\label{tab:rerank_sim}
		\footnotesize
		\vspace{-3mm}
		\begin{tabular}{|p{1.5cm}<{\centering}|c|c|c|p{0.7cm}<{\centering}|p{0.8cm}<{\centering}|}
			\hline
			Similarity     & MRR & Hit@1 & Hit@3 & Hit@5 & Hit@10  \\ \hline
			$Sim_m$*     &    0.382  &  0.263  &     0.449   &   0.522&     0.590                         \\ \hline
			$Sim_{func}$* &  0.297    &  0.194  & 0.343   &    0.410      & 0.502                        \\ \hline
			$Sim_{obj}$*   & 0.340   &  0.229 &   0.390  &   0.465      &    0.573                      \\ \hline
			$Sim_{iv}$*   &  0.383  &   0.271 &  0.447  &  0.520     &    0.592                       \\ \hline
			$Sim_{it}$*  &   0.370  &  0.251   &  0.437  &      0.510   &   0.592                     \\ \hline
			$Sim_{ot}$*   &   0.381  & 0.265   &  \textbf{0.451}   & \textbf{0.527}    &    0.580                     \\ \hline
			$Sim_{neig}$*     & \textbf{0.385}&    \textbf{0.273}  &   0.447  &  \textbf{0.527}  &  0.578                            \\ \hline
			%	All   & \textbf{0.385}&    \textbf{0.273} &   \textbf{0.447}  &  \textbf{0.527}  &  \textbf{0.578}                            \\ \hline
			All  & 0.384 &   0.267 &   0.449 &   \textbf{0.527}&    \textbf{0.594} \\ \hline
		\end{tabular}
	\end{table}
%\end{comment}








==> rq4_bak.tex <==
We compare the offline cost of \app under different scales to discuss the scalability of \app.
Table~\ref{tab:scale} shows the comparison of constructing cost for three API KGs, including a large-scale API KG, a medium-scale API KG, and a small-scale API KG (the KG constructed in RQ3~\ref{sec:rq3}).
Among them, \textit{Input}, \textit{Construct.}, \textit{Embed.}, and \textit{Infer.} represent the time on downloading JAR Files as input, API KG construction, API KG Embedding, and inferring analogical API methods for a query, respectively.
Although the number of entities increases by 2019 times from a small-scale API KG to a large-scale API KG, the time required for collecting inputs, API KG construction, and API KG embedding only increases by 386 times, 121 times, and 40 times, respectively.
Online inference time of \app is less than one second, which does not change with the scale of the API KG. 
Note that for new libraries, the steps of collection input, KG construction, KG embedding can all be incremental.
%Note that the online inference time of \app does not change much as the API KG grows, which improves the usability of \app.
\begin{table}[]
	%\scriptsize
	\centering
	\vspace{-4mm}
	\caption{Comparison of the Offline Cost of \app under Different Scales}
	\label{tab:scale}
	\footnotesize
	\vspace{-3mm}
	\begin{tabular}{|p{0.8cm}<{\centering}|c|c|c|p{0.8cm}<{\centering}|p{1.0cm}<{\centering}|p{0.7cm}<{\centering}|}
		\hline
		 Type & Library & Entity & Relation   & Input & Construct. & Embed. \\ \hline
		 Small    & 16&35K      &   2M        &     7m             &      49m          &       1.5h            \\ \hline
		 Medium  &    899& 2M     &   8M           &       1h           &     4h           &    6h           \\ \hline
		 Large &   35,773 & 72M     &   289M           &       45h           &     99h           &    60h          \\ \hline
	\end{tabular}
	\vspace{-7mm}
\end{table}

\subsubsection{Summary}
\app can scale with the increase of the number of libraries.
%\app is scalable by supporting the continuous expansion of new libraries in the API KG.



